Diversified Multiscale Graph Learning with Graph Self-Correction

Though the multiscale graph learning techniques have enabled advanced feature extraction frameworks, the classic ensemble strategy may show inferior performance while encountering the high homogeneity of the learnt representation, which is caused by the nature of existing graph pooling methods. To cope with this issue, we propose a diversified multiscale graph learning model equipped with two core ingredients: a graph self-correction (GSC) mechanism to generate informative embedded graphs, and a diversity boosting regularizer (DBR) to achieve a comprehensive characterization of the input graph. The proposed GSC mechanism compensates the pooled graph with the lost information during the graph pooling process by feeding back the estimated residual graph, which serves as a plug-in component for popular graph pooling methods. Meanwhile, pooling methods enhanced with the GSC procedure encourage the discrepancy of node embeddings, and thus it contributes to the success of ensemble learning strategy. The proposed DBR instead enhances the ensemble diversity at the graph-level embeddings by leveraging the interaction among individual classifiers. Extensive experiments on popular graph classification benchmarks show that the proposed GSC mechanism leads to significant improvements over state-of-the-art graph pooling methods. Moreover, the ensemble multiscale graph learning models achieve superior enhancement by combining both GSC and DBR.

==> Figure/diagram_multiscale.tex <==
\begin{figure} [t]
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.8\linewidth]{Figure/multiscale-demo.pdf}
  \caption{Diagram of multiscale graph learning.
 }
 \label{fig:diagram-multiscale}
 \vspace{-3mm}
\end{figure}

==> Table/tab-DiversityHelpEnsemble.tex <==
\begin{table}[t] %[hth]
\centering
% \vspace{0.5mm}
\caption{
        The effect of Diversity Regularizer on promoting the multiscale graph ensemble learning.
        }
\vspace{1mm}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|ccccc}
\toprule
     Method                                           & PROTEINS             & NCI1               & NCI109             \\ 
\midrule
    GSC-B (SAGPool)                            &  74.27$_{\pm0.80}$                  &  71.91$_{\pm0.93}$             &  71.69$_{\pm0.70}$     \\
    + Ensemble                                 &  74.47$_{\pm0.72}$ (-)              &  73.10$_{\pm0.69}$ (-)         &  72.13$_{\pm0.69}$  (-)    \\
    + Ensemble w. DPP                          &  74.71$_{\pm0.64}$  ($\uparrow$)    &  -                             &  72.54$_{\pm0.68}$  ($\uparrow$)(run)     \\
\midrule
    GSC-B (ASAP)                                &  74.39$_{\pm0.71}$                 &  74.52$_{\pm0.69}$               &  73.64$_{\pm0.49}$  \\
    + Ensemble                                  &  74.86$_{\pm0.51}$ (-)             &  74.93$_{\pm0.67}$               &  74.32$_{\pm0.47}$  (-)   \\
    + Ensemble w. DPP                           &  74.94$_{\pm0.51}$  ($\uparrow$)   &  -                               &  -               \\
% \hline
\bottomrule                     
\end{tabular}                           
}
\label{tab:effect-diversity-on-ensemble}
\vspace{-3mm}
\end{table}

==> Table/tab-append-GSChelp.tex <==
\begin{table*}[h] %[hth]
\centering
% \vspace{0.5mm}
\caption{
        The effect of Graph Self-Correction on improving performance of the ensemble strategy on the 6-layer GNN backbone. 
        }
\vspace{1mm}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{c|c|ccccc}
\toprule
  Layer &   Method             &     D\&D                              & PROTEINS                                  &  NCI1                         & NCI109                                        &   FRANKENSTEIN    \\ 
\midrule
 \multirow{4}{*}{6} &   SAGPool$^*$       &  73.34$_{\pm0.60}$ (-)                  &  73.34$_{\pm0.43}$ (-)                    &  70.67$_{\pm1.17}$  (-)               &  71.36$_{\pm0.12}$ (-)                 &  60.84$_{\pm0.85}$ (-)      \\
  &  + Ensemble        &  71.83$_{\pm0.82}$ (\green{$\downarrow$}) &  72.43$_{\pm1.28}$ (\green{$\downarrow$})   &  71.02$_{\pm0.43}$ (\red{$\uparrow$})  &  70.97$_{\pm1.18}$ (\green{$\downarrow$})   &  59.91$_{\pm0.56}$ (\green{$\downarrow$})     \\
\cmidrule{2-7}
  &  GSC-B (SAGPool)  &  75.35$_{\pm0.78}$  (-)                &  74.23$_{\pm0.28}$    (-)             &  71.73$_{\pm1.17}$ (-)      &  72.33$_{\pm0.36}$    (-)             &  61.67$_{\pm0.51}$ (-)    \\
  &  + Ensemble       &  75.58$_{\pm0.46}$ (\red{$\uparrow$})  &  74.75$_{\pm0.79}$ (\red{$\uparrow$})  &  72.01$_{\pm1.02}$  (\red{$\uparrow$}) &  73.07$_{\pm0.91}$ (\red{$\uparrow$})  &  62.19$_{\pm0.69}$  (\red{$\uparrow$})   \\
% \hline
\midrule
 \multirow{4}{*}{9} &   SAGPool$^*$       &  \urgent{TODO-Below} (-)                  &  73.34$_{\pm0.43}$ (-)                    &  70.67$_{\pm1.17}$  (-)               &  71.36$_{\pm0.12}$ (-)                 &  60.84$_{\pm0.85}$ (-)      \\
  &  + Ensemble        &  71.83$_{\pm0.82}$ (\green{$\downarrow$}) &  72.43$_{\pm1.28}$ (\green{$\downarrow$})   &  71.02$_{\pm0.43}$ (\red{$\uparrow$})  &  70.97$_{\pm1.18}$ (\green{$\downarrow$})   &  59.91$_{\pm0.56}$ (\green{$\downarrow$})     \\
\cmidrule{2-7}
  &  GSC-B (SAGPool)  &  75.35$_{\pm0.78}$  (-)                &  74.23$_{\pm0.28}$    (-)             &  71.73$_{\pm1.17}$ (-)      &  72.33$_{\pm0.36}$    (-)             &  61.67$_{\pm0.51}$ (-)    \\
  &  + Ensemble       &  75.58$_{\pm0.46}$ (\red{$\uparrow$})  &  74.75$_{\pm0.79}$ (\red{$\uparrow$})  &  72.01$_{\pm1.02}$  (\red{$\uparrow$}) &  73.07$_{\pm0.91}$ (\red{$\uparrow$})  &  62.19$_{\pm0.69}$  (\red{$\uparrow$})   \\
\bottomrule                     
\end{tabular}                           
}
\label{tab:append-GSC-on-ensemble}
% \vspace{-3mm}
\end{table*}

==> Table/tab-hyperparameter.tex <==
\begin{table}[h] %[hth]
\centering
% \vspace{0.5mm}
\caption{Hyper-parameter search range for multiscale graph learning model.}
\vspace{1mm}
\resizebox{0.35\linewidth}{!}{
\begin{tabular}{c|c}
\toprule
     Hyper-parameter        & Range               \\ 
\midrule
    Learning rate           & \{0.01, 0.005, 0.001\}   \\
    Hidden dimension        & \{16, 32, 64, 128\}                  \\
    Pooling ratio           & \{0.25, 0.5\}       \\
% \hline
\bottomrule                     
\end{tabular}                           
}
\label{tab:hyper-multiscale}  

% \vspace{-3mm}
\end{table}

\begin{table}[h] %[hth]
\centering
% \vspace{0.5mm}
\caption{Hyper-parameter search range for diversity boosting regularizer.}
\vspace{1mm}
\resizebox{0.31\linewidth}{!}{
\begin{tabular}{c|c}
\toprule
     Hyper-parameter        & Range               \\ 
\midrule
    $\gamma$ of gaussian kernel        & \{1, 5, 10\}   \\
    $\alpha$ of loss weight        & \{0.1, 1, 10\}                  \\
% \hline
\bottomrule                     
\end{tabular}                           
}
\label{tab:hyper-dbr}
% \vspace{-3mm}
\end{table}

==> Table/tab-misleading.tex <==
\begin{table}[h] %[hth]
\centering
% \vspace{0.5mm}
\caption{Test accuracy comparison of the ensemble strategy under different evaluation protocols.}
\vspace{1mm}
\resizebox{0.45\linewidth}{!}{
\begin{tabular}{c|cc}
\toprule
     Dataset: NCI1                     & Select-on-Validation             & Select-on-Test                      \\ 
\midrule
    SAGPool                     &  69.88 (-)               &  70.85 (-)      \\
    + Ensemble               &  69.61 ($\downarrow$)    &  72.00 ($\uparrow$)      \\
% \hline
\bottomrule                     
\end{tabular}                           
}
\label{tab:protocol-ensemble}
% \vspace{-3mm}
\end{table}
